Signaling in Posted Price Auctions

We study single-item single-unit Bayesian posted price auctions, where buyers arrive sequentially and their valuations for the item being sold depend on a random, unknown state of nature. The seller has complete knowledge of the actual state and can send signals to the buyers so as to disclose information about it. For instance, the state of nature may reflect the condition and/or some particular features of the item, which are known to the seller only. The problem faced by the seller is about how to partially disclose information about the state so as to maximize revenue. Unlike classical signaling problems, in this setting, the seller must also correlate the signals being sent to the buyers with some price proposals for them. This introduces additional challenges compared to standard settings. We consider two cases: the one where the seller can only send signals publicly visible to all buyers, and the case in which the seller can privately send a different signal to each buyer. As a first step, we prove that, in both settings, the problem of maximizing the seller's revenue does not admit an FPTAS unless P=NP, even for basic instances with a single buyer. As a result, in the rest of the paper, we focus on designing PTASs. In order to do so, we first introduce a unifying framework encompassing both public and private signaling, whose core result is a decomposition lemma that allows focusing on a finite set of possible buyers' posteriors. This forms the basis on which our PTASs are developed. In particular, in the public signaling setting, our PTAS employs some ad hoc techniques based on linear programming, while our PTAS for the private setting relies on the ellipsoid method to solve an exponentially-sized LP in polynomial time. In the latter case, we need a custom approximate separation oracle, which we implement with a dynamic programming approach.

==> contents/ex_intro.tex <==
\section{Example}
This example shows how the seller can increase their revenue through a signaling scheme in the case of multiple types of the receiver.
%
The set of state of nature is $\Theta=\{H,L\}$ that corresponds to a high-quality or low-quality item, respectively.
%
There is one sender and one receiver who share the same prior on the state of nature, that is $\mu=\{\mu_H=0.3,\mu_{L}=0.7\}$.
%
The receiver has two possible types, $k_1$ or $k_2$, (i.e., $\mathcal{K}=\{k_1,k_2\}$) and each type corresponds to a private valuation.
%
Type $k_1$ is associated to a valuation vector $\bm{v}=\{v_{H},v_{L}\}=\{\frac{3}{4},\frac{1}{4}\}$, while, type $k_2$ to a valuation vector $\bm{v}=\{1,0\}$.
%
The distribution over types of receiver $r$ is $D_r=\{\frac{1}{2},\frac{1}{2}\}$.
%
The seller fix a price $p$ for the item.
%
The available actions for buyers are to accept or refuse the offer (\emph{i.e.}, $\mathcal{A}=\{A,R\}$).



\begin{table}[h!]
	\begin{center}
		%	{\renewcommand{\arraystretch}{1.0}
		
		\begin{tabular}{r|c|l}
			& State H & State L \\
			& $\mu_{H}=0.3$ & $\mu_{L}=0.7$ \\
			\hline
			$A$ & p \quad   3/4 & p \quad  1/4    \\
			\hline
			$R$ & 0  \quad  0 & 0  \quad  0    \\
			\hline
		\end{tabular}
		
	\end{center}
	\caption{Payoff type $k_1$: left column is the sender, right column is the receiver}
	\label{table:payoff_k1}
\end{table}

\begin{table}[h!]
	\begin{center}
		%	{\renewcommand{\arraystretch}{1.0}
		
		\begin{tabular}{r|c|l}
			& State H & State L \\
			& $\mu_{H}=0.3$ & $\mu_{L}=0.7$ \\
			\hline
			$A$ & p \quad   1 & p \quad  0    \\
			\hline
			$R$ & 0  \quad  0 & 0  \quad  0    \\
			\hline
		\end{tabular}
		
	\end{center}
	\caption{Payoff type $k_2$: left column is the sender, right column is the receiver}
	\label{table:payoff_k2}
\end{table}

\textbf{No signaling scheme}

If the sender set price $p=0.3$ its expected utility is $\mathbb{E}[\mathcal{R}_s]=1/2*0.3+1/2*0.3=0.3$ because all the types play $A$.
If the sender set price $p=0.4$ its expected utility is $\mathbb{E}[\mathcal{R}_s]=1/2*0.4=0.2$ because type $k_1$ plays $A$, while type $k_2$ plays $R$ (because $\mathbb{E}[R_{k_2}]= 0.3$).
%
Therefore, seller set the revenue maximizing price \textcolor{blue}{$p=0.3$} and has $\mathbb{E}[\mathcal{R}_s]=\textcolor{orange}{0.3}$.

Notice that, in this case, the sender do not take advantage of his/her knowledge of the realized state of nature.

\textbf{With signaling scheme}

\begin{table}[h!]
	\begin{center}
		%	{\renewcommand{\arraystretch}{1.0}
		
		\begin{tabular}{r|c|l}
			& State H & State L \\
			\hline
			$s_{1}$ & 1 & 3/7    \\
			\hline
			$s_{2}$ & 0  & 4/7   \\
			\hline
		\end{tabular}
		
	\end{center}
	\caption{Signals}
	\label{table:signals_k}
\end{table}
\begin{table}[h!]
	\begin{center}
		%	{\renewcommand{\arraystretch}{1.0}
		
		\begin{tabular}{r|c|c|l}
			& State H & State L & $\textnormal{\textbf{w}}$\\
			\hline
			$\bm{\xi}^{s_1}$ & 1/2 & 1/2 & 3/5   \\
			\hline
			$\bm{\xi}^{s_2}$ & 0  & ~~1 & 2/5  \\
			\hline
		\end{tabular}
		
	\end{center}
	\caption{Posterior Beliefs}
	\label{table:posterior_beliefs_k}
\end{table}

The posterior beliefs in Table \ref{table:posterior_beliefs_k} are induced. When sending signal $s_2$, the sender set the revenue maximizing price \textcolor{blue}{$p=v^{k_1}_{L}=0.25$} and has $\mathbb{E}[\mathcal{R}_s]=v^{k_1}_{L} D_{L}^{k_1}=0.25 * 1/2 = 0.125$. When the signal is $s_1$, the seller set \textcolor{blue}{$p=0.5$} so that both the types accept and $\mathbb{E}[\mathcal{R}_s]=0.5$.
Therefore the final expected revenue of the sender is $\mathbb{E}[\mathcal{R}_s]=2/5 * 0.125 + 3/5 * 0.5 = \textcolor{orange}{0.35}$.


==> contents/extensions.tex <==
\section{extensions}

Number of state of natures exponential(come il paper che abbiamo letto)-->interessante

Known valuation--> dovrebbe avere algoritmo polinomiale

Distribuzioni dei diversi bidder correlate--> ritorniamo al problema bayesiano senza signaling che non riuscivamo a risolvere


distribuzioni dei buyers indipendenti per ogni stato di natura----> boooooooo

==> contents/notation.tex <==
\section{Thesis-Compliant Notation}

\paragraph{(Non-Bayesian) Posted Price Auctions}
\begin{itemize}
	\item $\mathcal{N} \coloneqq \{1, \ldots, n\}$ set of buyers, with $i \in \mathcal{N}$ denoting the $i$-th buyer in order of arrival.
	%
	\item $v_i \in [0,1]$ valuation of buyer $i \in \mathcal{N}$.
	%
	\item $\mathcal{V}_i$ distribution of buyers $i$'s valuations, supported on $[0,1]$.
	%
	\item $\mathcal{V} \coloneqq \{ \mathcal{V}_i \}_{i \in \mathcal{N}}$ distributions of valuations of all buyers.
	%
	\item ${p}_i \in [0,1]$ price proposed to buyer $i \in \mathcal{N}$.
	%
	\item $\textsc{Rev}$ expected revenue of the seller.
	%
\end{itemize}
\paragraph{Bayesian Posted Price Auctions}
\begin{itemize}
	\item $\Theta$ states of nature, with $|\Theta| \coloneqq d$.
	%
	\item ${v}_i \in [0,1]^d$ valuation of buyer $i \in \mathcal{N}$ in the Bayesian setting, with ${v}_i(\theta)$ denoting the valuation of the buyer when the state of nature is $\theta \in \Theta$.
	%
	\item $\mathcal{V}_i$ distribution of buyers $i$'s valuations in the Bayesian setting, supported on $[0,1]^d$.
	%
	\item $\mathcal{V} \coloneqq \{ \mathcal{V}_i \}_{i \in \mathcal{N}}$ distributions of valuations of all buyers in the Bayesian setting.\todo{\scriptsize Notice that notation is overloaded}
	%
	\item ${V} \in [0,1]^{n \times d}$ matrix of buyers' valuations, whose entries are defined as ${V}_{i,\theta} \coloneqq {v}_i(\theta)$ for all $i \in \mathcal{N}$ and $\theta \in \Theta$. Moreover, ${V}_i$ is the $i$-th row of ${V}$, that is ${V}_i = {v}_i^\top$.
	%
	\item ${\mu} \in \Delta^{|\Theta|}$ prior distribution over states of nature, with ${\mu}_{\theta}$ denoting the probability of state $\theta \in \Theta$.
\end{itemize}
\paragraph{Signaling Schemes and Payment Functions}
\begin{itemize}
	\item $\mathcal{S}_i$ signals reserved for buyer $i \in \mathcal{N}$.
	%
	\item $\mathcal{S} \coloneqq \bigtimes_{i \in \mathcal{N}} \mathcal{S}_i$ signal profiles, with $s = (s_1, \ldots, s_n) \in \mathcal{S}$ denoting that signal $s_i$ is sent to buyer $i$.
	%
	\item $\phi : \Theta \to \Delta^{|\mathcal{S}|}$ signaling scheme.
	\item ${\phi}_\theta \coloneqq \phi(\theta)$ probability distribution over signal profiles employed when the state is $\theta \in \Theta$, with $\phi_{\theta} (s)$ denoting the probability of drawing $s \in \mathcal{S}$. 
	\item ${\phi}_{i, \theta} \in \Delta^{|\mathcal{S}_i|}$ marginal probability distribution over signals of buyer $i \in \mathcal{N}$ when the state is $\theta \in \Theta$, with $\phi_{i,\theta}(s_i)$ denoting the probability of sending signal $s_i \in \mathcal{S}_i$; formally 
	\[
		{\phi}_{i, \theta}(s_i) \coloneqq \sum_{s' = (s_1', \ldots, s_n') \in \mathcal{S} : s_i' = s_i} {\phi}_\theta(s) \hspace{1cm} \forall s_i \in \mathcal{S}_i.
	\]
	%
	\item $p : \mathcal{S} \to [0,1]^n$ payment function.
	\item ${p}_s \coloneqq p(s)$ payments for a signal profile $s \in \mathcal{S}$, with $p_s(i)$ denoting the price proposed to buyer $i \in\mathcal{N}$.
	%
	\item ${\xi}_{i, s_i} \in \Delta^{|\Theta|}$ posterior belief of a buyer $i \in \mathcal{N}$ upon receiving signal $s_i \in \mathcal{S}_i$, with $\xi_{i,s_i}(\theta)$ denoting the probability of being in state $\theta \in \Theta$ according to the posterior belief; formally
	\[
		{\xi}_{i, s_i}(\theta)\coloneqq\frac{{\mu}_\theta {\phi}_{i, \theta}(s_i) }{\sum_{\theta'\in\Theta}{\mu}_{\theta'} {\phi}_{i, \theta'}(s_i) } \hspace{1cm} \forall \theta \in \Theta.
	\]
	%
	\item $\Xi_i \subseteq \Delta^{|\Theta|}$ possible posteriors of buyer $i \in \mathcal{N}$, formally $\Xi_i \coloneqq \left\{ {\xi}_{i, s_i} \mid s_i \in \mathcal{S}_i \right\}$.
	%
	\item $\Xi \coloneqq \bigtimes_{i \in \mathcal{N}} \Xi_i$ posterior profiles, with $\xi = ({\xi}_1, \ldots, {\xi}_n) \in \Xi$ denoting that buyer $i \in \mathcal{N}$ has posterior ${\xi}_i$.
	%
	\item $\xi_s \in \Xi$ posterior profile resulting from a signal profile $s \in \mathcal{S}$, formally $\xi_s = ({\xi}_{1, s_1}, \ldots, {\xi}_{n, s_n})$.
	%
	\item ${\gamma}_i \in \Delta^{|\Xi_i|}$ probability distribution over posterior beliefs of buyer $i \in \mathcal{N}$ induced by a signaling scheme  $\phi : \Theta \to \Delta^{|\mathcal{S}|}$, with $\gamma_i(\xi_i)$ denoting the probability of posterior $\xi_i \in \Xi_i$; formally 
	\[
		{\gamma}_i({\xi}_i)  \coloneqq \sum_{s_i \in \mathcal{S}_i: {\xi}_{i} = {\xi}_{i,s_i} } \sum_{\theta \in \Theta} {\mu}_\theta {\phi}_{i, \theta}(s_i) \hspace{1cm} \forall {\xi}_i \in \Xi_i.
	\]
\end{itemize}
\paragraph{Public Signaling}
\begin{itemize}
	\item A signaling scheme $\phi : \Theta \to \Delta^{|\mathcal{S}|}$ is public if: (1) $\mathcal{S}_i = \mathcal{S}_j$ for all $i, j \in \mathcal{N}$, and (2) for every $\theta \in \Theta$, $\boldsymbol{\phi}_\theta[s] > 0$ only for signal profiles $s \in \mathcal{S}$ such that $s_i = s_j$ for all $i, j \in \mathcal{N}$.
	%
	\item Since under a public signaling scheme $\phi : \Theta \to \Delta^{|\mathcal{S}|}$ all the buyers always share the same posterior belief (formally, for every $s \in \mathcal{S}$, it holds ${\xi}_{i, s_i} = {\xi}_{j, s_j}$ for all $i, j \in \mathcal{N}$), with an overload of notation we let ${\xi}_{s} \in \Delta^{|\Theta|}$ be the posterior belief of the buyers upon receiving signals specified by $s \in \mathcal{S}$.
	%
	\item $\textsc{Rev}(\mathcal{V},{p}, {\xi})$ expected revenue of the seller when all the buyers share the same posterior belief ${\xi} \in \Delta^{|\Theta|}$, given payments $p \in  [0,1]^n$.
	%
	\item $\textsc{Rev}_i(\mathcal{V},{p}, {\xi})$ expected revenue of the seller when all buyers $j \in \mathcal{N} : j < i$ preceding $i \in\mathcal{N}$ are excluded and all the remaining buyers share the same posterior belief ${\xi} \in \Delta^{|\Theta|}$, given payments $p \in  [0,1]^n$.\todo{\scriptsize Notice that there is an overload of notation}
	%
	\item Utility of a pair $\phi : \Theta \to \Delta^{|\mathcal{S}|}$ and $p : \mathcal{S} \to [0,1]^n$:
	\[
		\sum_{\theta \in \Theta} {\mu}_\theta \sum_{s \in \mathcal{S}} {\phi}_\theta(s) \textsc{Rev}(\mathcal{V},{p}_s, {\xi}_s)
	\]
\end{itemize}
\paragraph{Private Signaling}
\begin{itemize}
	\item $\textsc{Rev}(\mathcal{V},{p}, \xi)$ expected revenue of the seller when the buyers' posterior beliefs are those specified by $\xi \in \Xi$, given payments $p \in  [0,1]^n$.
	%
	\item Utility of a pair $\phi : \Theta \to \Delta^{|\mathcal{S}|}$ and $p : \mathcal{S} \to [0,1]^n$:
	\[
	\sum_{\theta \in \Theta} {\mu}_\theta \sum_{s \in \mathcal{S}} {\phi}_\theta(s) \textsc{Rev}(\mathcal{V},{p}_s, {\xi}_s).
	\]
\end{itemize}
\paragraph{Discrete Payment Vectors}
\begin{itemize}
	\item $P_b \coloneqq \left\{ \frac{x}{b} \mid x = 0, \ldots, b \right\}$ discrete set of payments of size $b \in \mathbb{N}$.
	%
	\item $\mathcal{P}_b \coloneqq \bigtimes_{i \in \mathcal{N}} P_b$ discrete set of payment vectors.
\end{itemize}

